Topological Portfolio Selection and Optimization

Modern portfolio optimization is centered around creating a low-risk portfolio with extensive asset diversification. Following the seminal work of Markowitz, optimal asset allocation can be computed using a constrained optimization model based on empirical covariance. However, covariance is typically estimated from historical lookback observations, and it is prone to noise and may inadequately represent future market behavior. As a remedy, information filtering networks from network science can be used to mitigate the noise in empirical covariance estimation, and therefore, can bring added value to the portfolio construction process. In this paper, we propose the use of the Statistically Robust Information Filtering Network (SR-IFN) which leverages the bootstrapping techniques to eliminate unnecessary edges during the network formation and enhances the network's noise reduction capability further. We apply SR-IFN to index component stock pools in the US, UK, and China to assess its effectiveness. The SR-IFN network is partially disconnected with isolated nodes representing lesser-correlated assets, facilitating the selection of peripheral, diversified and higher-performing portfolios. Further optimization of performance can be achieved by inversely proportioning asset weights to their centrality based on the resultant network.

==> main <==
%%% -*-BibTeX-*-
%%% Do NOT edit. File created by BibTeX with style
%%% ACM-Reference-Format-Journals [18-Jan-2012].

\begin{thebibliography}{30}

%%% ====================================================================
%%% NOTE TO THE USER: you can override these defaults by providing
%%% customized versions of any of these macros before the \bibliography
%%% command.  Each of them MUST provide its own final punctuation,
%%% except for \shownote{}, \showDOI{}, and \showURL{}.  The latter two
%%% do not use final punctuation, in order to avoid confusing it with
%%% the Web address.
%%%
%%% To suppress output of a particular field, define its macro to expand
%%% to an empty string, or better, \unskip, like this:
%%%
%%% \newcommand{\showDOI}[1]{\unskip}   % LaTeX syntax
%%%
%%% \def \showDOI #1{\unskip}           % plain TeX syntax
%%%
%%% ====================================================================

\ifx \showCODEN    \undefined \def \showCODEN     #1{\unskip}     \fi
\ifx \showDOI      \undefined \def \showDOI       #1{#1}\fi
\ifx \showISBNx    \undefined \def \showISBNx     #1{\unskip}     \fi
\ifx \showISBNxiii \undefined \def \showISBNxiii  #1{\unskip}     \fi
\ifx \showISSN     \undefined \def \showISSN      #1{\unskip}     \fi
\ifx \showLCCN     \undefined \def \showLCCN      #1{\unskip}     \fi
\ifx \shownote     \undefined \def \shownote      #1{#1}          \fi
\ifx \showarticletitle \undefined \def \showarticletitle #1{#1}   \fi
\ifx \showURL      \undefined \def \showURL       {\relax}        \fi
% The following commands are used for tagged output and should be
% invisible to TeX
\providecommand\bibfield[2]{#2}
\providecommand\bibinfo[2]{#2}
\providecommand\natexlab[1]{#1}
\providecommand\showeprint[2][]{arXiv:#2}

\bibitem[Aste(2022)]%
        {aste2020topological}
\bibfield{author}{\bibinfo{person}{Tomaso Aste}.}
  \bibinfo{year}{2022}\natexlab{}.
\newblock \showarticletitle{Topological regularization with information
  filtering networks}.
\newblock \bibinfo{journal}{\emph{Information Sciences, arXiv:2005.04692}}
  (\bibinfo{year}{2022}).
\newblock


\bibitem[Aste and Matteo(2017)]%
        {CompNet4}
\bibfield{author}{\bibinfo{person}{T. Aste} {and} \bibinfo{person}{T. Matteo}.}
  \bibinfo{year}{2017}\natexlab{}.
\newblock \showarticletitle{Sparse Causality Network Retrieval from Short Time
  Series}.
\newblock \bibinfo{journal}{\emph{Complex.}}  \bibinfo{volume}{2017}
  (\bibinfo{year}{2017}), \bibinfo{pages}{4518429:1--4518429:13}.
\newblock


\bibitem[Barfuss et~al\mbox{.}(2016)]%
        {CompNet7}
\bibfield{author}{\bibinfo{person}{Wolfram Barfuss},
  \bibinfo{person}{Guido~Previde Massara}, \bibinfo{person}{T. Di~Matteo},
  {and} \bibinfo{person}{Tomaso Aste}.} \bibinfo{year}{2016}\natexlab{}.
\newblock \showarticletitle{Parsimonious modeling with information filtering
  networks}.
\newblock \bibinfo{journal}{\emph{Physical Review E}} \bibinfo{volume}{94},
  \bibinfo{number}{6} (\bibinfo{date}{Dec} \bibinfo{year}{2016}).
\newblock
\showISSN{2470-0053}
\urldef\tempurl%
\url{https://doi.org/10.1103/physreve.94.062306}
\showDOI{\tempurl}


\bibitem[Briola and Aste(2022)]%
        {Briola2022DependencySI}
\bibfield{author}{\bibinfo{person}{Antonio Briola} {and}
  \bibinfo{person}{Tomaso Aste}.} \bibinfo{year}{2022}\natexlab{}.
\newblock \showarticletitle{Dependency structures in cryptocurrency market from
  high to low frequency}.
\newblock


\bibitem[Dees et~al\mbox{.}(2019)]%
        {Dees2019PortfolioCA}
\bibfield{author}{\bibinfo{person}{Bruno~Scalzo Dees}, \bibinfo{person}{L.
  Stankovi{\'c}}, \bibinfo{person}{Anthony~G. Constantinides}, {and}
  \bibinfo{person}{Danilo~P. Mandic}.} \bibinfo{year}{2019}\natexlab{}.
\newblock \showarticletitle{Portfolio Cuts: A Graph-Theoretic Framework to
  Diversification}.
\newblock \bibinfo{journal}{\emph{ICASSP 2020 - 2020 IEEE International
  Conference on Acoustics, Speech and Signal Processing (ICASSP)}}
  (\bibinfo{year}{2019}), \bibinfo{pages}{8454--8458}.
\newblock


\bibitem[Friedman et~al\mbox{.}(2008)]%
        {CompNet9}
\bibfield{author}{\bibinfo{person}{J. Friedman}, \bibinfo{person}{T. Hastie},
  {and} \bibinfo{person}{R. Tibshirani}.} \bibinfo{year}{2008}\natexlab{}.
\newblock \showarticletitle{Sparse inverse covariance estimation with the
  graphical lasso.}
\newblock \bibinfo{journal}{\emph{Biostatistics}}  \bibinfo{volume}{9 3}
  (\bibinfo{year}{2008}), \bibinfo{pages}{432--41}.
\newblock


\bibitem[Konstantinov et~al\mbox{.}(2020)]%
        {Konstantinov2020ANA}
\bibfield{author}{\bibinfo{person}{Gueorgui~S. Konstantinov},
  \bibinfo{person}{Andreas Chorus}, {and} \bibinfo{person}{Jonas Rebmann}.}
  \bibinfo{year}{2020}\natexlab{}.
\newblock \showarticletitle{A Network and Machine Learning Approach to Factor,
  Asset, and Blended Allocation}.
\newblock


\bibitem[Kruskal(1956)]%
        {CompNet10}
\bibfield{author}{\bibinfo{person}{Joseph~B. Kruskal}.}
  \bibinfo{year}{1956}\natexlab{}.
\newblock \showarticletitle{On the shortest spanning subtree of a graph and the
  traveling salesman problem}.
\newblock


\bibitem[Ledoit and Wolf(2003)]%
        {Ledoit2003HoneyIS}
\bibfield{author}{\bibinfo{person}{Olivier Ledoit} {and}
  \bibinfo{person}{Michael Wolf}.} \bibinfo{year}{2003}\natexlab{}.
\newblock \showarticletitle{Honey, I Shrunk the Sample Covariance Matrix}.
\newblock \bibinfo{journal}{\emph{Capital Markets: Asset Pricing \& Valuation}}
  (\bibinfo{year}{2003}).
\newblock


\bibitem[Ledoit and Wolf(2004)]%
        {Ledoit2004AWE}
\bibfield{author}{\bibinfo{person}{Olivier Ledoit} {and}
  \bibinfo{person}{Michael Wolf}.} \bibinfo{year}{2004}\natexlab{}.
\newblock \showarticletitle{A well-conditioned estimator for large-dimensional
  covariance matrices}.
\newblock \bibinfo{journal}{\emph{Journal of Multivariate Analysis}}
  \bibinfo{volume}{88} (\bibinfo{year}{2004}), \bibinfo{pages}{365--411}.
\newblock


\bibitem[Li et~al\mbox{.}(2013)]%
        {Li2013UnveilingCB}
\bibfield{author}{\bibinfo{person}{Ming-Xia Li}, \bibinfo{person}{Zhi-Qiang
  Jiang}, \bibinfo{person}{Wen-Jie Xie}, \bibinfo{person}{Xiong Xiong},
  \bibinfo{person}{Wei Zhang}, {and} \bibinfo{person}{Wei‐Xing Zhou}.}
  \bibinfo{year}{2013}\natexlab{}.
\newblock \showarticletitle{Unveiling correlations between financial variables
  and topological metrics of trading networks: Evidence from a stock and its
  warrant}.
\newblock \bibinfo{journal}{\emph{Physica A-statistical Mechanics and Its
  Applications}}  \bibinfo{volume}{419} (\bibinfo{year}{2013}),
  \bibinfo{pages}{575--584}.
\newblock


\bibitem[Li et~al\mbox{.}(2019)]%
        {Li2019PortfolioOB}
\bibfield{author}{\bibinfo{person}{Yan Li}, \bibinfo{person}{Xiongfei Jiang},
  \bibinfo{person}{Yue Tian}, \bibinfo{person}{Sai-Ping Li}, {and}
  \bibinfo{person}{Bo Zheng}.} \bibinfo{year}{2019}\natexlab{}.
\newblock \showarticletitle{Portfolio optimization based on network topology}.
\newblock \bibinfo{journal}{\emph{Physica A: Statistical Mechanics and its
  Applications}} (\bibinfo{year}{2019}).
\newblock


\bibitem[Lohre et~al\mbox{.}(2014)]%
        {Lohre2014TheUO}
\bibfield{author}{\bibinfo{person}{Harald Lohre}, \bibinfo{person}{Jochen
  Papenbrock}, {and} \bibinfo{person}{Muddit Poonia}.}
  \bibinfo{year}{2014}\natexlab{}.
\newblock \showarticletitle{The Use of Correlation Networks in Parametric
  Portfolio Policies}.
\newblock \bibinfo{journal}{\emph{Econometric Modeling: Capital Markets - Risk
  eJournal}} (\bibinfo{year}{2014}).
\newblock


\bibitem[Mantegna(1999)]%
        {Mantegna1999HierarchicalSI}
\bibfield{author}{\bibinfo{person}{Rosario~N. Mantegna}.}
  \bibinfo{year}{1999}\natexlab{}.
\newblock \showarticletitle{Hierarchical structure in nancial markets}.
\newblock


\bibitem[{Markowitz}(1952)]%
        {Markowitz}
\bibfield{author}{\bibinfo{person}{H. {Markowitz}}.}
  \bibinfo{year}{1952}\natexlab{}.
\newblock \showarticletitle{Portfolio Selection}.
\newblock \bibinfo{journal}{\emph{The Journal of Finance}} \bibinfo{volume}{7},
  \bibinfo{number}{1} (\bibinfo{year}{1952}).
\newblock


\bibitem[Massara and Aste(2019a)]%
        {CompNet6}
\bibfield{author}{\bibinfo{person}{Guido~Previde Massara} {and}
  \bibinfo{person}{Tomaso Aste}.} \bibinfo{year}{2019}\natexlab{a}.
\newblock \showarticletitle{Learning Clique Forests}.
\newblock \bibinfo{journal}{\emph{ArXiv}}  \bibinfo{volume}{1905.02266}
  (\bibinfo{year}{2019}).
\newblock


\bibitem[Massara and Aste(2019b)]%
        {Massara2019LearningCF}
\bibfield{author}{\bibinfo{person}{Guido~Previde Massara} {and}
  \bibinfo{person}{Tomaso Aste}.} \bibinfo{year}{2019}\natexlab{b}.
\newblock \showarticletitle{Learning Clique Forests}.
\newblock \bibinfo{journal}{\emph{ArXiv}}  \bibinfo{volume}{abs/1905.02266}
  (\bibinfo{year}{2019}).
\newblock


\bibitem[Massara et~al\mbox{.}(2017)]%
        {CompNet5}
\bibfield{author}{\bibinfo{person}{Guido~Previde Massara}, \bibinfo{person}{T.
  Matteo}, {and} \bibinfo{person}{T. Aste}.} \bibinfo{year}{2017}\natexlab{}.
\newblock \showarticletitle{Network Filtering for Big Data: Triangulated
  Maximally Filtered Graph}.
\newblock \bibinfo{journal}{\emph{ArXiv}}  \bibinfo{volume}{abs/1505.02445}
  (\bibinfo{year}{2017}).
\newblock


\bibitem[Ne{\v{s}}et{\v{r}}il et~al\mbox{.}(2001)]%
        {nevsetvril2001otakar}
\bibfield{author}{\bibinfo{person}{Jaroslav Ne{\v{s}}et{\v{r}}il},
  \bibinfo{person}{Eva Milkov{\'a}}, {and} \bibinfo{person}{Helena
  Ne{\v{s}}et{\v{r}}ilov{\'a}}.} \bibinfo{year}{2001}\natexlab{}.
\newblock \showarticletitle{Otakar Boruvka on minimum spanning tree problem
  Translation of both the 1926 papers, comments, history}.
\newblock \bibinfo{journal}{\emph{Discrete mathematics}} \bibinfo{volume}{233},
  \bibinfo{number}{1-3} (\bibinfo{year}{2001}), \bibinfo{pages}{3--36}.
\newblock


\bibitem[Onnela et~al\mbox{.}(2003)]%
        {Onnela2003DynamicsOM}
\bibfield{author}{\bibinfo{person}{Jukka-Pekka Onnela},
  \bibinfo{person}{Anirban Chakraborti}, \bibinfo{person}{Kimmo~K. Kaski},
  \bibinfo{person}{J{\'a}nos Kert{\'e}sz}, {and} \bibinfo{person}{Antti~J.
  Kanto}.} \bibinfo{year}{2003}\natexlab{}.
\newblock \showarticletitle{Dynamics of market correlations: taxonomy and
  portfolio analysis.}
\newblock \bibinfo{journal}{\emph{Physical review. E, Statistical, nonlinear,
  and soft matter physics}}  \bibinfo{volume}{68 5 Pt 2}
  (\bibinfo{year}{2003}), \bibinfo{pages}{056110}.
\newblock


\bibitem[Peralta and Zareei(2016)]%
        {Peralta2016ANA}
\bibfield{author}{\bibinfo{person}{Gustavo Peralta} {and}
  \bibinfo{person}{Abalfazl Zareei}.} \bibinfo{year}{2016}\natexlab{}.
\newblock \showarticletitle{A Network Approach to Portfolio Selection}.
\newblock \bibinfo{journal}{\emph{Econometric Modeling: Capital Markets -
  Portfolio Theory eJournal}} (\bibinfo{year}{2016}).
\newblock


\bibitem[Pozzi et~al\mbox{.}(2013)]%
        {Pozzi2013SpreadOR}
\bibfield{author}{\bibinfo{person}{Francesca Pozzi},
  \bibinfo{person}{Tiziana~Di Matteo}, {and} \bibinfo{person}{Tomaso Aste}.}
  \bibinfo{year}{2013}\natexlab{}.
\newblock \showarticletitle{Spread of risk across financial markets: better to
  invest in the peripheries}.
\newblock \bibinfo{journal}{\emph{Scientific Reports}}  \bibinfo{volume}{3}
  (\bibinfo{year}{2013}).
\newblock


\bibitem[Prim(1957)]%
        {CompNet11}
\bibfield{author}{\bibinfo{person}{Robert~C. Prim}.}
  \bibinfo{year}{1957}\natexlab{}.
\newblock \showarticletitle{Shortest connection networks and some
  generalizations}.
\newblock \bibinfo{journal}{\emph{Bell System Technical Journal}}
  \bibinfo{volume}{36} (\bibinfo{year}{1957}), \bibinfo{pages}{1389--1401}.
\newblock


\bibitem[Procacci and Aste(2021)]%
        {Procacci2021PortfolioOW}
\bibfield{author}{\bibinfo{person}{Pier~Francesco Procacci} {and}
  \bibinfo{person}{Tomaso Aste}.} \bibinfo{year}{2021}\natexlab{}.
\newblock \showarticletitle{Portfolio optimization with sparse multivariate
  modeling}.
\newblock \bibinfo{journal}{\emph{Journal of Asset Management}}
  \bibinfo{volume}{23} (\bibinfo{year}{2021}), \bibinfo{pages}{445 -- 465}.
\newblock


\bibitem[Saef et~al\mbox{.}(2022)]%
        {Saef2022RegimebasedIS}
\bibfield{author}{\bibinfo{person}{Danial Saef}, \bibinfo{person}{Yuanrong
  Wang}, {and} \bibinfo{person}{Tomaso Aste}.} \bibinfo{year}{2022}\natexlab{}.
\newblock \showarticletitle{Regime-based Implied Stochastic Volatility Model
  for Crypto Option Pricing}.
\newblock \bibinfo{journal}{\emph{ArXiv}}  \bibinfo{volume}{abs/2208.12614}
  (\bibinfo{year}{2022}).
\newblock


\bibitem[Sensoy and Tabak(2014)]%
        {Sensoy2014DynamicST}
\bibfield{author}{\bibinfo{person}{Ahmet Sensoy} {and}
  \bibinfo{person}{Benjamin~Miranda Tabak}.} \bibinfo{year}{2014}\natexlab{}.
\newblock \showarticletitle{Dynamic spanning trees in stock market networks:
  The case of Asia-Pacific}.
\newblock \bibinfo{journal}{\emph{Physica A-statistical Mechanics and Its
  Applications}}  \bibinfo{volume}{414} (\bibinfo{year}{2014}),
  \bibinfo{pages}{387--402}.
\newblock


\bibitem[Stuart and Markowitz(1959)]%
        {Stuart1959PortfolioSE}
\bibfield{author}{\bibinfo{person}{Alan~L. Stuart} {and}
  \bibinfo{person}{Harry~M. Markowitz}.} \bibinfo{year}{1959}\natexlab{}.
\newblock \showarticletitle{Portfolio Selection: Efficient Diversification of
  Investments}.
\newblock \bibinfo{journal}{\emph{A Quarterly Journal of Operations Research}}
  \bibinfo{volume}{10} (\bibinfo{year}{1959}), \bibinfo{pages}{253}.
\newblock


\bibitem[Telesford et~al\mbox{.}(2011)]%
        {CompNet8}
\bibfield{author}{\bibinfo{person}{Qawi~K. Telesford}, \bibinfo{person}{S.
  Simpson}, \bibinfo{person}{J. Burdette}, \bibinfo{person}{S. Hayasaka}, {and}
  \bibinfo{person}{P. Laurienti}.} \bibinfo{year}{2011}\natexlab{}.
\newblock \showarticletitle{The Brain as a Complex System: Using Network
  Science as a Tool for Understanding the Brain}.
\newblock \bibinfo{journal}{\emph{Brain connectivity}}  \bibinfo{volume}{1 (4)}
  (\bibinfo{year}{2011}), \bibinfo{pages}{295--308}.
\newblock


\bibitem[Tumminello et~al\mbox{.}(2005)]%
        {CompNet3}
\bibfield{author}{\bibinfo{person}{M. Tumminello}, \bibinfo{person}{T. Aste},
  \bibinfo{person}{T. Di~Matteo}, {and} \bibinfo{person}{R.~N. Mantegna}.}
  \bibinfo{year}{2005}\natexlab{}.
\newblock \showarticletitle{A tool for filtering information in complex
  systems}.
\newblock \bibinfo{journal}{\emph{Proceedings of the National Academy of
  Sciences}} \bibinfo{volume}{102}, \bibinfo{number}{30}
  (\bibinfo{year}{2005}), \bibinfo{pages}{10421--10426}.
\newblock
\showISSN{0027-8424}
\urldef\tempurl%
\url{https://doi.org/10.1073/pnas.0500298102}
\showDOI{\tempurl}
\showeprint{https://www.pnas.org/content/102/30/10421.full.pdf}


\bibitem[Wang and Aste(2021)]%
        {Wang2021DynamicPO}
\bibfield{author}{\bibinfo{person}{Yuanrong Wang} {and} \bibinfo{person}{Tomaso
  Aste}.} \bibinfo{year}{2021}\natexlab{}.
\newblock \showarticletitle{Dynamic portfolio optimization with inverse
  covariance clustering}.
\newblock \bibinfo{journal}{\emph{Expert Syst. Appl.}}  \bibinfo{volume}{213}
  (\bibinfo{year}{2021}), \bibinfo{pages}{118739}.
\newblock


\end{thebibliography}

